A Survey of the State-of-the-Art Parallel Multiple Sequence Alignment Algorithms on Multicore Systems

Evolutionary modeling applications are the best way to provide full information to support in-depth understanding of evaluation of organisms. These applications mainly depend on identifying the evolutionary history of existing organisms and understanding the relations between them, which is possible through the deep analysis of their biological sequences. Multiple Sequence Alignment (MSA) is considered an important tool in such applications, where it gives an accurate representation of the relations between different biological sequences. In literature, many efforts have been put into presenting a new MSA algorithm or even improving existing ones. However, little efforts on optimizing parallel MSA algorithms have been done. Nowadays, large datasets become a reality, and big data become a primary challenge in various fields, which should be also a new milestone for new bioinformatics algorithms. This survey presents four of the state-of-the-art parallel MSA algorithms, TCoffee, MAFFT, MSAProbs, and M2Align. We provide a detailed discussion of each algorithm including its strengths, weaknesses, and implementation details and the effectiveness of its parallel implementation compared to the other algorithms, taking into account the MSA accuracy on two different datasets, BAliBASE and OXBench.

==> text/Abstract.tex <==
\begin{abstract}
Among all `big data' research issues, the veracity challenge, which refers to the precision and accuracy of the data, has not received as much attention. Traditionally, it has been well known that problems related to data quality, such as incomplete, redundant, inconsistent, and noisy data pose a major challenge to data mining and data analysis. Particularly, we note that existing methods for handling missing values cannot scale to larger datasets. In other words, this particular veracity challenge has been addressed, but not in context of also handling volume (and possibly the velocity) challenge of `big data'.
This paper focuses on speeding up the missing values imputation process using the bitmap indexing technique. The research takes two directions: first, the bitmap indexing is used to directly access the required records for the imputation method (i.e., Direct Access Imputation (DAI)). Second, the bitmap indexing technique is used for missing value estimation using the pre-generated bitmap indexing vectors without accessing the dataset itself (i.e., Bitmap-Based Imputation (BBI)). Both approaches have been evaluated using different real and synthetic datasets, and four common imputation algorithms. We show how our bitmap-based methods can accelerate data mining classification of incomplete data while also maintaining precision.

\end{abstract}


==> text/related.tex <==
Clustal Series:
The Clustal series [3] are the most widely used tools for global multiple sequence alignment. The first Clustal program combined the progressive alignment strategy with dynamic programming using a guided tree. Then ClustalW incorporated a number of improvements to the alignment algorithm, including sequence weighting, position specific gap penalties and the automatic choice of a suitable residue comparison matrix.
In 2001 [4] Dmitri Mikhailo proposes a parallel version of clustal the three stages of clustal were paralyzed in first stage pair-wise (PW) in this stage because of each pair-wise comparison is independent so it can be easy to parallel this stage. In the second stage guide tree (GT)the most time wasted when calculating the minimum matrix This can be done in parallel by calculating and saving the minimum element of each row concurrently and then using the saved minimum row elements to find the minimum element of the entire matrix. The third stage progressive alignment (PA) in this stage during the final PA, the original code makes calls to the score (i,j)  function within a loop.  Although the loop itself cannot be parallelized, the calculation of each score (i,j)  can be recomputed in parallel. The parallel version shows speedups of up to 10x when running Clustal W on 16 CPUs and significantly reduces the time required for data analysis.
In 2003 [5] James Cheetham proposes a new parralel version pCLUSTAL is another parallel version  of  ClustalW  using  MPI.  In  contrast  to  the  commercial  SGI  parallel Clausal  version,  which  requires  an  expensive  SGI  multiprocessor  system,  pCLUSTAL  can  be  run  on  a  range  of distributed  and  shared  memory  parallel  machines,  from  high-end  parallel  multiprocessors  to  PC  clusters,  to  simple networks  of  workstations  and  achieve  relative  speedup.  Another  acceleration  of  ClustalW have  been  developed  in  on  multiprocessor  SMP  cluster  using  a  hybrid  MPI/OpenMP  method  with  mixed  fine  and  coarse  grained parallelization  approach  in  the  third  stage.  A  speedup  of  80  and  9.2  was  obtained  for  the  first  and  third  stages respectively,  and  an  overall  speedup  of  35  using  40  nodes  and  80  processors.
MUSCLE Series:
MUSCLE [6] is a widely used program. It has achieved a higher rank in accuracy and a faster speed compared to ClustalW and T-Coffee. It includes fast distance estimation using kmer counting; progressive alignment using a new profile function called the log-expectation score and refinement using tree-dependent restricted partitioning
In 2006 [7] Xi Deng proposed a paralleled MUSCLE algorithm which are parallelized with different OpenMP paradigms. MUSCLE uses two round implementation of progressive alignment. The first round alignment (FRA) is a basic alignment. The result used in second round. The first round consists of the basic steps of progressive alignment. The second round consists of two primary modules (PMC) primary matrix computation and (CT) consistency transformation. They notice that most of time running on the three modules (FRA, PMC, CT) ,so they think about Paralleled of these modules. In the first module FRA each parent nodes depends on its leaves so the parallel step can be difficult here they used a queue to insert tasks in it. In the two other modules they assign every processor with same amount of computation on nodes pairs. The performance of   parallel MUSCLE is conducted on a 16-way Intel Xeon shared-memory multiprocessor system. It has 16 x86 processors running at 3.0GHz, 4 levels of cache with each 4MB L4 cache shared amongst 4 CPUs. The sizes of the L1, L2 and L3 caches are 8K, 512K and 4MB respectively. As for the interconnect, the system uses two 4x4 crossbars. They use Intel 8.0 C++ OpenMP compiler tool chain to generate the executables with options-O3 -ipo -openmp, to enable the high levels of compiler optimizations. The experimental results show that their parallel implementation scales pretty well on 16-way system (15.2x speedup on dataset 100). By comparing with the performance of a 4-way system, they conclude that large L3 cache as well as combined L4 cache can sharply reduce the last level cache miss rate, which is the bottleneck of MUSCLE, and thus do help to improve the scalability performance of MUSCLE.
MAFFT Series:
MAFFT [8] is another popular MSA program. It included two novel techniques that reduce the CPU time. It identified homologous regions by the fast Fourier transform.
In 2010 [9] katoh proposal maff at program with parallization using posix threads library they paralyzed the steps of mafft algorithm, firstly they paralyze the stage of all-to-all comparison by using multiple threads to process different pair using alignment simultaneously and independently with little loss of cpu time .secondly in the stage of progressive alignment group to group alignment calculations are performed along with guide tree. They cannot make a parallization in this stage because each part depend on each other. So the efficiency of parallization in this stage is low. finally iterative refinement process the alignment divided into two sub-alignment and then the two sub-alignment are realigned. They used best first and simple hill-climbing parallization strategy this alignment achieved a peak speedup of 10 times with different random numberona16 corepc(4 × Quad-Core AMD Opteron Processor 8378).
T-COFFEE Series:
T-Coffee [10] was the first MSA software that uses a consistency-based objective function optimized using progressive alignment. It tries to maximize the score between the final multiple alignment and a library of pair-wise residue-by residue scores derived from a mixture of local and global pair-wise alignments.
In 2010 [11] The parallization is controlled with  $multi_core=templates_jobs_relax_msa$. Where the flag consists of four different keyword that control the alignment step(1)template selection template are always identified by running a blast against an appropriate database.(2) library computation :in this step parallization is achieved by grapping the alignment tasks into number of individual jobs equal to the number of available process jobs are then submitted and the output is merged.(3) library extension: score for aligning every residue pair.(4) progressive alignment: the progressive alignment stage align sequence two by two. The parallization done by separately processing all the independent nodes the medium instance.

